Designing Gaze Analytics for ELA Instruction: A User-Centered Dashboard with Conversational AI Support

Eye-tracking offers rich insights into student cognition and engagement, but remains underutilized in classroom-facing educational technology due to challenges in data interpretation and accessibility. In this paper, we present the iterative design and evaluation of a gaze-based learning analytics dashboard for English Language Arts (ELA), developed through five studies involving teachers and students. Guided by user-centered design and data storytelling principles, we explored how gaze data can support reflection, formative assessment, and instructional decision-making. Our findings demonstrate that gaze analytics can be approachable and pedagogically valuable when supported by familiar visualizations, layered explanations, and narrative scaffolds. We further show how a conversational agent, powered by a large language model (LLM), can lower cognitive barriers to interpreting gaze data by enabling natural language interactions with multimodal learning analytics. We conclude with design implications for future EdTech systems that aim to integrate novel data modalities in classroom contexts.

==> figures/latest_dashboard.tex <==
\begin{figure}[h]
  \centering

  % \renewcommand{\thesubfigure}{}
  \captionsetup[subfloat]{labelformat=empty}  % Completely removes (a), (b), ...
  
  \subfloat[]{%
    \includegraphics[width=0.48\textwidth]{imgs/teacher_dashboard.png}%
  }
  \hfill
  \subfloat[]{%
    \includegraphics[width=0.48\textwidth]{imgs/student_dashboard.png}%
  }
  \caption{\textbf{}}
  \label{fig:dashboard}
\end{figure}

